Dynamic Packet Aggregation to Solve Performance Anomaly in 802.11 Wireless Networks

In the widely used 802.11 standard, the so called performance anomaly is a well known issue. Several works have tried to solve this problem by introducing mechanisms such as packet fragmentation, backoff adaptation, or packet aggregation during a fixed time interval. In this paper, we propose a novel approach solving the performance anomaly problem by packet aggregation using a dynamic time interval, which depends on the busy time of the wireless medium. Our solution differs from other proposition in the literature because of this dynamic time interval, which allows increasing fairness, reactivity, and in some cases efficiency. In this article, we emphasize the performance evaluation of our proposal.

==> abstract.tex <==
% The Abstract
In the widely used 802.11 standard, the so called \emph{performance
anomaly}  is a well known issue. Several works have tried to solve
this problem by introducing  mechanisms such as packet fragmentation,
backoff adaptation, or packet aggregation during a fixed time
interval. 
In this paper, we propose a novel approach solving the
performance anomaly problem by packet aggregation using a dynamic
time interval, which depends on the busy time of the
wireless medium. 
Our solution differs from other proposition in the
literature because of this dynamic time interval, which allows 
increasing fairness, reactivity, and in some cases efficiency. 
In this article, we emphasize the performance evaluation of our 
proposal.

